Improving Compositional Attribute Binding in Text-to-Image Generative Models via Enhanced Text Embeddings

Text-to-image diffusion-based generative models have the stunning ability to generate photo-realistic images and achieve state-of-the-art low FID scores on challenging image generation benchmarks. However, one of the primary failure modes of these text-to-image generative models is in composing attributes, objects, and their associated relationships accurately into an image. In our paper, we investigate compositional attribute binding failures, where the model fails to correctly associate descriptive attributes (such as color, shape, or texture) with the corresponding objects in the generated images, and highlight that imperfect text conditioning with CLIP text-encoder is one of the primary reasons behind the inability of these models to generate high-fidelity compositional scenes. In particular, we show that (i) there exists an optimal text-embedding space that can generate highly coherent compositional scenes showing that the output space of the CLIP text-encoder is sub-optimal, and (ii) the final token embeddings in CLIP are erroneous as they often include attention contributions from unrelated tokens in compositional prompts. Our main finding shows that significant compositional improvements can be achieved (without harming the model's FID score) by fine-tuning only a simple and parameter-efficient linear projection on CLIP's representation space in Stable-Diffusion variants using a small set of compositional image-text pairs.

==> sections/introduction.tex <==
\newcommand{\earlystop}{\textsc{Switch-Off}}

\begin{figure*}
\centering
\includegraphics[width=\textwidth]{figures/main_figure.png}
\vspace{-17pt}
\caption{Overview of our analysis and proposed methods. The figure identifies two sources of errors in Stable Diffusion's inability to generate compositional prompts: (i) erroneous attention contribution in CLIP (minor) and (ii) sub-optimal CLIP text embedding (major). We propose a window-based linear projection (\wb{}), applying linear projection to a token’s surrounding window to enhance embeddings.
% \SF{the linear projection seems to be applied on a subset of tokens; perhaps improve the visualization; also suggest to write the text tokens in black to make it more readable}
}

\label{fig:main_fig}
\end{figure*}

\section{Introduction}
Text-to-image diffusion-based generative models~\citep{DBLP:journals/corr/abs-2112-10752, podell2023sdxl, dalle, saharia2022photorealistic} have achieved photo-realistic image generation capabilities on user-defined text prompts. 
However, recent studies~\citep{huang2023t2icompbench} reveal that text-to-image models struggle with maintaining high fidelity when handling simple compositional prompts, such as those consisting of attributes, objects, and their associated relations (\eg, ``{\it a red book and a yellow vase}'').  This hinders the use of these generative models in various creative scenarios where the end-user wants to generate scenes that accurately reflect the composition and relationships specified in the prompt.

Existing approaches~\citep{chefer2023attendandexcite, feng2023layoutgpt, agarwal2023astar, wang2023compositional} explore various strategies to enhance compositionality in text-to-image models.
These methods primarily focus on modifying cross-attention maps by utilizing bounding box annotations and performing optimizations in the latent space during inference. Recent advancements, such as fine-tuning the UNet~\citep{huang2023t2icompbench}, have also demonstrated improvements in compositionality.
However, the {\it core reasons} behind compositionality failures remain poorly understood. Gaining insights into these root causes is crucial for developing more effective approaches to augment these models with enhanced compositional capabilities.

In our paper, we investigate the potential causes of compositional attribute binding failures in text-to-image generative models, where the model fails to correctly associate descriptive attributes (such as color, shape, or texture) with the corresponding objects in the generated images. We identify two key sources of error:
(i) {\it Erroneous attention contributions in CLIP output token embeddings}: We observe that output token embeddings in CLIP have significant attention contributions from irrelevant tokens, thereby introducing errors in generation. To explore this, we compare the internal attention contributions in CLIP for compositional prompts with the T5 text encoder, known for its stronger compositionality. Quantitative analysis shows that T5 exhibits fewer erroneous attention contributions than CLIP, indicating a potential reason for its superior compositionality.
(ii) {\it Sub-optimality of CLIP output space for compositional prompts}: We find out that there exists an alternative text-embedding space capable of generating highly coherent images from compositional prompts. This indicates that the current CLIP output space is inherently sub-optimal. 
Specifically, optimizing CLIP's text embeddings, while keeping the Stable Diffusion UNet frozen, converges to a more effective embedding space, enabling better compositional image generation.
These findings highlight that refining the output space of the CLIP text encoder could play a critical role in enhancing compositionality.

% To circumvent this problem, we use the Stable-Diffusion UNet, but optimize for text-embeddings (with CLIP initialization) for images with compositional scenes. We first find out that there exists a text-embedding space capable of generating highly coherent compositional scenes for various attributes (e.g., {\it color, texture, shape, spatial position}) which highlights that the existing CLIP output space is sub-optimal. Furthermore, we study the model internals of the CLIP text-encoder for compositional prompts and show that the output token embeddings have attention contributions from irrelevant tokens, thereby introducing errors. Together, these results highlight that the output space of the CLIP text-encoder can be further improved to augment text-to-image models with improved compositionality. 

%% Contributions for improvements %%
% Building on our observations regarding the deficiencies of the CLIP, we show that we can improve the output space of the CLIP text-encoder to better align it with the optimal space by applying a \textit{simple} linear projection on top of the CLIP (see Figure~\ref{fig:main_fig}).

Building on our observations about the deficiencies of CLIP and identifying its text-embedding space as \textit{a core issue} in compositional attribute binding, we explore augmenting diffusion models with a lightweight module to enhance the text-encoder's output and improve compositionality. Remarkably, a simple linear projection achieves significant improvements, comparable or superior to full fine-tuning of CLIP or training more complex networks on top of it. We demonstrate that this linear projection effectively aligns the CLIP text-encoder’s output with a more optimal embedding space (see Figure~\ref{fig:main_fig}), leading to significantly stronger compositional performances.

In particular, we introduce Window-based Compositional Linear Projection ($\wb$), a \textit{lightweight} fine-tuning method that significantly improves the model’s performance on compositional prompts (Figure~\ref{fig:prompts_examples}), achieving results comparable to or surpassing existing methods. 
Additionally, $\wb$ preserves the model's overall performance, maintaining high fidelity on clean prompts as evidenced by a low FID score, while offering a solution that is both \textit{parameter efficient} and \textit{speed efficient}. This ensures robust compositional capabilities without compromising the model's general effectiveness.
% We further conduct an study on the parameter space used for improving CLIP outputs, comparing full fine-tuning and last-layer fine-tuning. Both approaches achieve improvements comparable to our method, highlighting its effectiveness and parameter efficiency. Additionally, we analyze token-level contributions to compositionality, identifying critical tokens whose improved embeddings lead to enhanced generation.



% Fine-tuning a subset of components of the diffusion model can result in an increase in the FID score for clean prompts.  While fine-tuning only a linear projection partially mitigates this, we find that applying it over all the time steps results in an increase in the FID score. To address this, we propose \earlystop{}, a strategy where $\wb$ is applied only during the initial steps of the generation process and switched off for the remaining steps. This approach allows the model to establish a coherent compositional structure in the early stages—critical for compositional prompts—while preserving clean accuracy for standard prompts. By relying on the original text encoder rather than the projected one during the later steps, \earlystop{} ensures high-quality generation across diverse prompt types.

In summary, our contributions are as follows:
\begin{itemize}
    \item We perform an in-depth analysis of the reasons behind compositionality failures in text-to-image generative models, with a particular focus on investigating the attribute binding aspect of compositionality. We highlight two key reasons contributing to these failures.
    \item Building on our observations, we propose $\wb$ as an enhancement for SD v1.4, SD v2, SDXL, SD v3, DeepFloyd, and PixArt-$\alpha$. This method significantly improves the models' compositional attribute binding, while preserving accuracy on standard prompts.
    We observe improvements of $16.18\%, 15.15\%$, and $9.51\%$ on SD v1.4, $14.35\%, 11.14\%$, and $6\%$ on SD v2, $20.31\%, 13.4\%$, and $5\%$ on SDXL, and $14.16\%$, $9.82\%$, and $2.63\%$ on PixArt-$\alpha$ in VQA scores across color, texture, and shape datasets, respectively.
    Our method outperforms or matches existing baselines in VQA scores, while achieving a superior FID score. It requires \textit{fewer parameters for optimization} and enables \textit{faster inference}, making it both efficient and effective. Extensive evaluations with T2I-CompBench, TIFA, and human studies validate our method's effectiveness.
    
\end{itemize}


% Overall, our paper provides quantitative evidence elucidating the compositional challenges within text-to-image models and strong baselines to mitigate such issues.
%\kr{@Samyadeep please read the intro. I think if don't go for t5 or unet finetuning -- we can make the paper more specific by saying we aim to understand the role of text-encoder.} \sbb{Edited the intro accordingly.}

\input{table_of_figures_tex_files/prompts_examples}
